Direct Bound-Electron $g$ factor Difference Measurement with Coupled Ions

The quantum electrodynamic (QED) description of light-and-matter interaction is one of the most fundamental theories of physics and has been shown to be in excellent agreement with experimental results. Specifically, measurements of the electronic magnetic moment (or $g$ factor) of highly charged ions (HCI) in Penning traps can provide a stringent probe for QED, testing the Standard model in the strongest electromagnetic fields. When studying the difference of isotopes, even the intricate effects stemming from the nucleus can be resolved and tested as, due to the identical electron configuration, many common QED contributions do not have to be considered. Experimentally however, this becomes quickly limited, particularly by the precision of the ion masses or the achievable magnetic field stability. Here we report on a novel measurement technique that overcomes both of these limitations by co-trapping two HCIs in a Penning trap and measuring the difference of their $g$ factors directly. The resulting correlation of magnetic field fluctuations leads to drastically higher precision. We use a dual Ramsey-type measurement scheme with the ions locked on a common magnetron orbit, separated by only a few hundred micrometres, to extract the coherent spin precession frequency difference. We have measured the isotopic shift of the bound electron $g$ factor of the neon isotopes of $^{20}$Ne$^{9+}$ and $^{22}$Ne$^{9+}$ to 0.56 parts-per-trillion ($5.6 \cdot 10^{-13}$) precision relative to their $g$ factors, which is an improvement of more than two orders of magnitude compared to state-of-the-art techniques. This resolves the QED contribution to the nuclear recoil for the very first time and accurately validates the corresponding theory. Furthermore, the agreement with theory allows setting constraints for a fifth-force, resulting from Higgs-portal-type dark-matter interactions.

==> Methods/NP_IS_Ne1.tex <==

%\documentclass[a4paper,10pt,twocolumn]{article}
%
%\setlength{\topmargin}{0cm}
%\setlength{\headheight}{0.4cm}
%\setlength{\headsep}{0.8cm}
%\setlength{\footskip}{1cm}
%\setlength{\textwidth}{17.5cm}
%\setlength{\textheight}{25cm}
%\setlength{\voffset}{-1.5cm}
%\setlength{\hoffset}{-0.5cm}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}

%\usepackage{graphicx}
%\usepackage[font=footnotesize,format=plain,labelfont=bf,up]{caption}
%\usepackage{subcaption}
%\usepackage{amstext}
%\usepackage{amsmath}			
%\usepackage{amssymb}
%\usepackage{wasysym}
%\usepackage{mathrsfs}
%\usepackage{setspace}
%\usepackage[utf8]{inputenc}
%\usepackage[british]{babel}     
%\usepackage{tabularx}				
%\usepackage{psfrag}
%\usepackage{siunitx}
%\usepackage[explicit,toctitles,pagestyles]{titlesec}
%\usepackage{pifont}
%\usepackage{csquotes}
%\usepackage{varwidth}
%\usepackage[style=nature, sorting=none,maxnames=3, firstinits=true, uniquename=init, sorting=none, url=false,isbn=false,eprint=false,texencoding=utf8,bibencoding=utf8, autocite=superscript,backend=biber]{biblatex}
%\usepackage{color}
%\usepackage{xcolor}
%\usepackage{titletoc}
%\usepackage{tikz}
%\usepackage[compat=1.1.0]{tikz-feynman}
%\usepackage{tikz-3dplot} 
%\tdplotsetmaincoords{60}{110}
%\pgfmathsetmacro{\rvec}{.8}
%\pgfmathsetmacro{\thetavec}{30}
%\pgfmathsetmacro{\phivec}{60}
%\usetikzlibrary{decorations.pathmorphing}
%\usetikzlibrary{shapes}

%\definecolor{link}{rgb}{0,0,.75}
%\definecolor{cite}{rgb}{.75,0,0}
%\definecolor{url}{rgb}{0,.75,0}
%\usepackage[pdftex,colorlinks=false,pdfstartview=FitV,linkbordercolor=link,citebordercolor=cite,urlbordercolor=url,hyperindex=true,hyperfigures=false]{hyperref}


%\setlength{\parindent}{0pt}

\subsection*{Setting Limits on New physics}
\label{sec:newPhysEnergy}
Measuring the $g$ factor allows for high-precision access to the properties of very tightly bound electrons, and hence to short-range Physics, including potential New Physics. Bounds on New Physics can be set with isotope shift data on the $g$ factor of H-like Ne. The Higgs portal mechanism, in particular, involves the mixing of a new (massive) scalar boson, the relaxion, with the Higgs boson. It has been proposed as a solution to the long-standing electroweak hierarchy problem~\cite{EightPage}, and the relaxion is a dark matter candidate~\cite{RelaxionDark}. Constraints on this proposed extension of the Standard Model (SM) can be set with cosmological data, as well as with particle colliders, beam dumps, and also with smaller, high-precision experiments (see, e.g., Ref.~\cite{PossibleForces} and references therein). The most common approach in atomic physics is to search for deviations from linearity on experimental isotope shift data in a so-called King plot analysis~\cite{PossibleForces,HiggsLikeAtomic,ProbingIS,FifthForce,FlambaumIso,LinXPCa}, which can be a sign of New Physics, although non-linearities can also happen within the SM~\cite{FlambaumIso,VladimirKing,FifthForceG,NonLinXPYb}, which limits the bounds which can be set on New Physics parameters. Here, we present constraints on New Physics from data on a single isotope pair.

The influence of Higgs Portal relaxions (scalar bosons) on atoms can be expressed~\cite{PossibleForces,ProbingIS,FifthForce,FlambaumIso} by a Yukawa-type potential (often called `fifth force') exerted by the nucleus on the atomic electrons:
\begin{equation} \label{eq:HPPotential}
  V_{\mathrm{HP}}\left(\mathbf{r}\right)=-\hbar c\,\alpha_{\mathrm{HP}}\,A\,\frac{\mathrm{e}^{-\frac{m_\phi c}{\hbar}\left|\mathbf{r}\right|}}{\left|\mathbf{r}\right|},
\end{equation}
where $m_\phi$ is the mass of the scalar boson, $\alpha_{\mathrm{HP}}=y_ey_n/4\pi$ is the Higgs portal coupling constant, with $y_e$ and $y_n$ the coupling of the boson to the electrons and the nucleons, respectively, and $A$ is the nuclear mass number. Yukawa potentials naturally arise when considering hypothetical new forces mediated by massive particles. The corresponding correction to the H-like $g$ factor is given by~\cite{FifthForceG}
\begin{multline} \label{eq:GNP}
  g_{\mathrm{HP}}=-\frac{4}{3}\alpha_{\mathrm{HP}}\,A\,\frac{\left(Z\alpha\right)}{\gamma}\,\left(1+\frac{m_\phi}{2Z\alpha m_e}\right)^{-2\gamma}\\
  \times\left[1+2\gamma-\frac{2\gamma}{1+\frac{m_\phi}{2Z\alpha m_e}}\right],
\end{multline}
where $\gamma=\sqrt{1-\left(Z\alpha\right)^2}$. The mass scale of the hypothetical new boson is not known~\cite{PossibleForces}, apart from the upper bound $m_\phi<60~\mathrm{GeV}$. In the small boson mass regime $m_\phi\ll Z\alpha m_e$, the contribution to the $g$ factor simplifies to
\begin{equation} \label{eq:GNPLight}
  g_{\mathrm{HP}}=-\frac{4}{3}\alpha_{\mathrm{HP}}\,A\,\frac{\left(Z\alpha\right)}{\gamma},\qquad m_\phi\ll Z\alpha m_e.
\end{equation}
In the large boson mass regime $m_\phi\gg Z\alpha m_e$, on the other hand, we obtain
\begin{multline} \label{eq:GNPHeavy}
  g_{\mathrm{HP}}=-\frac{4}{3}\alpha_{\mathrm{HP}}\,A\,\frac{\left(Z\alpha\right)\left(1+2\gamma\right)}{\gamma}\left(\frac{m_\phi}{2Z\alpha m_e}\right)^{-2\gamma},\\ m_\phi\gg Z\alpha m_e.
\end{multline}
\begin{center}
\begin{table} [tb]
\begin{center}
\def\arraystretch{1.25}
\begin{tabular}{c|c|c}
\hline
\hline
\multicolumn{1}{c}{Contribution} &
\multicolumn{1}{c}{Value (unc.)} &
\multicolumn{1}{c}{Ref.} \\
\hline
Leading Recoil & $1.33255\left[-8\right]$ &TW,\cite{RecoilAllOrders}\\
Relat. Leading Size & $1.66(11)\left[-10\right]$ &TW,\cite{ShabaevSize}\\
\hline
Higher-Order Recoil & $-7.65(4)\left[-12\right]$ &TW,\cite{EidesGrotch}\\
Higher-Order Size & $-4.06(40)\left[-13\right]$ &TW,\cite{FNSGHigher}\\
Finite Size Recoil & $-6.42(4)\left[-14\right]$ &TW,\cite{VladimirKing}\\
Radiative Recoil & $-1.03(2)\left[-11\right]$ &TW,\cite{ShabaevReview}\\
Radiative Finite Size & $<1\left[-12\right]$ &\cite{RadiativeNuclSize}\\
Deformation & $<1\left[-13\right]$ &\cite{NuDefNiklas}\\
Polarisation & $<2\left[-12\right]$ &TW,\cite{FifthForceG}\\
\hline
\hline
\end{tabular}
\end{center}
\caption{Various contributions to the \textsuperscript{20-22}Ne\textsuperscript{19+} $g$ factor isotope shift. Uncertainties are indicated between round brackets, powers of 10 between square brackets. TW: this work. \label{tab:IsoShift}}
\end{table}
\end{center}
We can set bounds on the New Physics coupling constant by comparing the measured and calculated values of the $g$-factor isotope shift (see Ref.~\cite{FifthForceG}, and also Ref.~\cite{CoulombHidden} for an implementation of the same idea with transition frequencies in atomic systems). Uncertainties from theory are a source of limitation in this approach. The SM contributions to the isotope shift of the $g$ factor of H-like Ne are given in Table~\ref{tab:IsoShift}, as calculated in this work based on the approaches developed in the indicated references. As can be seen, the largest theoretical uncertainty comes from the leading finite nuclear size correction, and is due to the limited knowledge of nuclear radii (the uncertainty on the finite nuclear size correction due to the choice of the nuclear model is negligible at this level of precision). We note that the standard source for these nuclear radii is data on X-ray transitions in muonic atoms~\cite{NuclRadiiUpdate}. In the NP relaxion scenario, the energy levels of these muonic atoms is also corrected by the relaxion exchange. Another source of root-mean-square charge radii and their differences is optical spectroscopy. The electronic transitions involved are far less sensitive to hypothetical NP than muonic X-ray transitions. The radius difference between \textsuperscript{20}Ne and \textsuperscript{22}Ne extracted from optical spectroscopy~\cite{NeonIsoShift} agrees with the one determined from muonic atom data within the respective uncertainties, which shows that NP need not be taken into account to extract nuclear radii from these experiments at their level of precision. To conclude, for our purposes, hypothetical contributions from NP do not interfere with the interpretation of muonic atom data for the extraction of nuclear radii. 

Taking $\Delta g_{\mathrm{theo}}^{AA'}=1.1\times10^{-11}$ as the theoretical error on the isotope shift, it can be seen from Eq.~(\ref{eq:GNPLight}) that this corresponds to an uncertainty of $\Delta y_ey_n\sim7.1\times10^{-10}$ in the small boson mass regime $m_\phi\ll Z\alpha m_e$, which is weaker than the currently most stringent bound coming from atomic physics~\cite{SpinIndep}. In the large boson mass regime $m_\phi\gg Z\alpha m_e$, on the other hand, we obtain bounds more stringent than those of Ref.~\cite{LinXPCa}, and almost identical with those of Ref.~\cite{SpinIndep}, thanks to two favourable factors. First, the nuclear charge $Z$ in Eq.~(\ref{eq:GNPHeavy}) is somewhat larger than the screened effective charge perceived by the Ca\textsuperscript{+} valence electron, and larger than the charge of the H and He nuclei, which also enter the scaling of the bound obtained with these respective ions~\cite{FifthForce}. Second, when carrying out a King analysis as done in Ref.~\cite{LinXPCa}, one works with two different transition frequencies, and the leading term in the hypothetical New Physics contribution in the large boson mass regime, which is the equivalent of the r.h.s. of Eq.~(\ref{eq:GNPHeavy}), is cancelled out in the nonlinearity search, due to its proportionality to the leading finite nuclear size correction~\cite{FifthForce}, leaving the next term, which scales as $\left(m_\phi/\left(2Z\alpha m_e\right)\right)^{-1-2\gamma}$, as the first non-vanishing contribution. In the present case, the $g$ factor of a single electronic state is considered (for a single isotope pair), and this cancellation does not occur. This leads to competitive bounds in the large boson mass regime with the simple $g$-factor isotope shift of H-like ions, as shown in Fig.~\ref{fig:exclusion} (where we used the exact result, Eq.~(\ref{eq:GNP})). We compare our bounds on the coupling constant $y_ey_n=4\pi\alpha_{\mathrm{HP}}$, to the bounds obtained in Refs.~\cite{LinXPCa,SpinIndep}, through isotope shift measurements in Ca\textsuperscript{+}, and H and He (we did not reproduce one of the bounds obtained in Ref.~\cite{SpinIndep}, which rests on the assumption of no muonic coupling to the relaxion), as well as to the bounds obtained through a combination of neutron scattering and free-electron $g$-factor data. We also indicate bounds that can be derived through measurement of $g$ factors of single ions: Si\textsuperscript{13+} from the measurement of Ref.~\cite{Sturm11}, and C\textsuperscript{5+} from the measurement of Ref.~\cite{Sturm14} combined with the mass measurement of Ref.~\cite{MassHD}.%, and Ne\textsuperscript{9+} from a projected determination at ALPHATRAP.\\
In the large boson mass regime $m_\phi\gg Z\alpha m_e$, we can set bounds on the New Physics coupling constant that improve by several orders of magnitude on the bounds obtained in Ref.\cite{LinXPCa}. For very high boson masses, the combined constraints from neutron scattering and the free $g$ factor drop off, and the bound obtained from He-like Ne $g$ factor isotope shift data becomes more competitive. In the $m_e<m_\phi<10^3m_e$ range, competitive constraints are also available from beam dump and meson decay experiments, while in the $10^3m_e<m_\phi<10^5m_e$ range, constraints come from collider experiments. Constraints obtained from beam dump, meson decay and collider experiments are placed on the mixing angle $\sin\theta_{\mathrm{HP}}$ between the Higgs boson and the relaxion in the Higgs portal scenario\cite{RHMix}. The coupling constants $\alpha_{\mathrm{Higgs}}$ corresponding to Higgs-boson exchange, and $\alpha_{\mathrm{HP}}$, are related through $\alpha_{\mathrm{HP}}=\alpha_{\mathrm{Higgs}}\sin\theta_{\mathrm{HP}}$\cite{HiggsLikeAtomic}. Although SM predictions exist for $\alpha_{\mathrm{Higgs}}$, these have not been tested stringently by collider experiments~\cite{HiggsLikeAtomic}, so that bounds on $\sin\theta_{\mathrm{HP}}$ do not necessarily translate univocally into bounds on $\alpha_{\mathrm{HP}}$. Bounds on $\alpha_{\mathrm{HP}}$ can be obtained indirectly, by combining bounds on $\sin\theta_{\mathrm{HP}}$ from meson decay~\cite{RHMix} with bounds on $\alpha_{\mathrm{Higgs}}$ from collider data~\cite{HiggsLikeAtomic}. In the  $m_e<m_\phi<10^3m_e$ range, they translate to bounds $y_ey_n=4\pi\alpha_{\mathrm{HP}}$ of order $10^{-6}$. Our results are hence of specific interest for setting bounds directly on the relaxion (Higgs portal) couplings, which has not been done to our knowledge with beam dump experiments. Nevertheless, for the heaviest regime $10^3m_e<m_\phi<10^5m_e$, we expect Higgs portal contributions to the $g$ factor to become smaller than contributions due to Higgs boson exchange, so that no bounds can be set on the Higgs portal for such relaxion masses.

In Fig.~\ref{fig:exclusion}, we also indicate projected bounds that could be obtained from isotope shift measurements of the $g$ factors of both H-like and Li-like Ne, as well as Ar. Combining both measurements allows the approximate cancellation of the leading finite nuclear size corrections through considering a weighted difference \cite{WDiffVeryOld,GFactorAlpha} of H-like and Li-like $g$ factors. On the basis of our earlier discussion of the domination of theoretical uncertainties by the uncertainty on the leading finite nuclear size correction (also see Table \ref{tab:IsoShift}), the interest of this approach is readily understood. Our calculations indicate that Ar is in the optimal range for setting bounds on $\alpha_{\mathrm{HP}}$ with this approach. The weighted difference approach is not preferred in the large boson mass regime, however, because the bound then scales as $\left(m_\phi/\left(2Z\alpha m_e\right)\right)^{1+2\gamma}$ as it does in the framework of King analysis.


